Are the observed gaps in protoplanetary discs caused by growing planets?

Recent detailed observations of protoplanetary discs revealed a lot of sub-structures which are mostly ring-like. One interpretation is that these rings are caused by growing planets. These potential planets are not yet opening very deep gaps in their discs. These planets instead form small gaps in the discs to generate small pressure bumps exterior to their orbits that stop the inflow of the largest dust particles. In the pebble accretion paradigm, this planetary mass corresponds to the pebble isolation mass, where pebble accretion stops and efficient gas accretion starts. We perform planet population synthesis via pebble and gas accretion including type-I and type-II migration. In the first stage of our simulations, we investigate the conditions necessary for planets to reach the pebble isolation mass and compare their position to the observed gaps. We find that in order to match the gap structures 2000 M E in pebbles is needed, which would be only available for the most metal rich stars. We then follow the evolution of these planets for a few My to compare the resulting population with the observed exoplanet populations. Planet formation in discs with these large amounts of pebbles result in mostly forming gas giants and only very little super-Earths, contradicting observations. This leads to the conclusions that either (i) the observed discs are exceptions, (ii) not all gaps in observed discs are caused by planets or (iii) that we miss some important ingredients in planet formation related to gas accretion and/or planet migration.

==> ucs.tex <==
%%
%% This is file `ucs.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% ucs.dtx  (with options: `ucs.sty')
%% 
%% Copyright 2001 Dominique Unruh  <unruh@ut.ee>
%% Copyright 2013 Wolfgang Jeltsch <wolfgang@cs.ioc.ee>
%% 
%% This program is provided under the terms of the LaTeX Project Public License with some
%% modifications. See the file LICENSE for information.
%% 
\catcode`\@11
\ifx\@gobble\undefined\def\@gobble#1{}\fi
\ifx\@gobbletwo\undefined\def\@gobbletwo#1#2{}\fi
\ifx\@gobblethree\undefined\def\@gobblethree#1#2#3{}\fi
\ifx\@gobblefour\undefined\def\@gobblefour#1#2#3#4{}\fi
\ifx\@firstofone\undefined\def\@firstofone#1{#1}\fi
\ifx\@tempcnta\undefined\csname newcount\endcsname\@tempcnta\fi
\ifx\@tempcntb\undefined\csname newcount\endcsname\@tempcntb\fi
\ifx\@testopt\undefined
  \def\@testopt#1#2{%
    \@ifnextchar[{#1}{#1[{#2}]}}\fi
\ifx\@protected@testopt\undefined\def\@protected@testopt{\expandafter\@testopt\@gobble}\fi
\let\@let@token\relax
\ifx\@ifnextchar\undefined
  \def\@ifnextchar#1#2#3{%
    \let\reserved@d=#1%
    \def\reserved@a{#2}%
    \def\reserved@b{#3}%
    \futurelet\@let@token\@ifnch}\fi
\ifx\@ifnch\undefined
  \def\@ifnch{%
    \ifx\@let@token\@sptoken
      \let\reserved@c\@xifnch
    \else
      \ifx\@let@token\reserved@d
        \let\reserved@c\reserved@a
      \else
        \let\reserved@c\reserved@b
      \fi
    \fi
    \reserved@c}\fi
\ifx\@inputcheck\undefined\newread\@inputcheck\fi
\ifx\IfFileExists\undefined
\long\def\IfFileExists#1#2#3{%
  \openin\@inputcheck#1 %SPACE
  \ifeof\@inputcheck\def\reserved@a{#3}%
  \else\closein\@inputcheck\def\reserved@a{#2}%
  \fi
  \reserved@a}%
\fi
\ifx\InputIfFileExists\undefined
\long\def\InputIfFileExists#1#2{%
  \IfFileExists{#1}{#2\input #1 }}
\fi
\ifx\protect\undefined\let\protect\relax\fi
\ifx\@typeset@protect\undefined\let\@typeset@protect\relax\fi
\ifx\IeC\undefined\def\IeC{\ifx\protect\@typeset@protect
  \expandafter\@firstofone\else\noexpand\IeC\fi}\fi
\def\unicode@knownoptions{}
\def\XDeclareUnicodeOption#1#2#3#4#5{%
  \expandafter\let\csname ifUnicodeOption#2\endcsname\iffalse
  \expandafter\def\csname UnicodeOption#2true%
    \expandafter\endcsname\expandafter{%
      \expandafter\let\csname ifUnicodeOption#2\endcsname\iftrue}%
  \expandafter\def\csname UnicodeOption#2false%
    \expandafter\endcsname\expandafter{%
      \expandafter\let\csname ifUnicodeOption#2\endcsname\iffalse}%
  \expandafter\def\csname @unicode@option@#2\endcsname{%
    #3\uni@activate@option{#2}{}{#4}{#5}}%
  \expandafter\def\csname @unicode@option@no#2\endcsname{%
    #3\uni@activate@option{#2}{no}{#4}{#5}}%
  \ifx~#1~\else\LinkUnicodeOptionToPkg{#2}{#1}\fi
  \let\uc@tempa\\\let\\\relax
  \edef\unicode@knownoptions{\\{#2}\unicode@knownoptions}%
  \let\\\uc@tempa
  }%
\let\uc@newcommand\def
\uc@newcommand\DeclareUnicodeOption{\@protected@testopt\DeclareUnicodeOption\DeclareUnicodeOption@{}}
\uc@newcommand\DeclareUnicodeOption@[#1]#2{%
  \XDeclareUnicodeOption{#1}{#2}{}{}{}}%
\uc@newcommand\uc@errormsg#1#2{%
  \ifx\PackageError\undefined
    {\newlinechar`\^^J\def\MessageBreak{^^J}%
      \errhelp{#2}\errmessage{Package ucs: #1}}%
  \else
    \PackageError{ucs}{#1}{#2}%
  \fi
}%
\uc@newcommand\uc@warnmsg#1{%
  \ifx\PackageWarning\undefined
    {\newlinechar`\^^J\def\MessageBreak{^^J}%
      \message{Package ucs: #1\MessageBreak}}%
  \else
    \PackageWarning{ucs}{#1}%
  \fi
}%
\def\uni@activate@option#1#2#3#4#5{%
  \ifx\uni@dataloaded\undefined
  \global\expandafter\def\csname @unicode@option@#1\endcsname##1{%
    \csname UnicodeOption#1true\endcsname
    \expandafter\def\csname uo-prio-#1\endcsname{##1}#3}%
  \global\expandafter\def\csname @unicode@option@no#1\endcsname##1%
    {\csname UnicodeOption#1false\endcsname#4}%
  \global\expandafter\let\csname uni@active@#1\endcsname1%
  \csname @unicode@option@#2#1\endcsname{#5}\else
  \uc@errormsg{Option #1 must be activated or deactivated %SPACE
    at least once in the preamble before using it in the document}{%
    For optimization causes I must know all %SPACE
    options before loading any unicode data.\MessageBreak
    Try e.g. #1 or no#1 as package option to ucs.}\fi}
\def\LinkUnicodeOptionToPkg#1#2{%
  \AtBeginDocument{\@ifpackageloaded{#2}{\SetUnicodeOption{#1}}{}}}%
\uc@newcommand\SetUnicodeOption{\@protected@testopt\SetUnicodeOption\SetUnicodeOption@{100}}
\uc@newcommand\SetUnicodeOption@[#1]#2{%
  \edef\uc@temp@a{@unicode@option@#2}%
  \expandafter\ifx\csname\uc@temp@a\endcsname\relax
    \PackageError{ucs}{Unknown unicode option #2}{}%
  \else
    \csname\uc@temp@a\endcsname{#1}%
  \fi}
\ifx\ProvidesPackage\undefined\else
\ProvidesPackage{ucs}[2013/05/11 v2.2 UCS: Unicode input support]%
\fi
\ifx\@@input\undefined\input uni-global.def \else\input{uni-global.def}\fi
\DeclareUnicodeOption{fasterrors}
\DeclareUnicodeOption{warnunknown}
\DeclareUnicodeOption{graphics}
\DeclareUnicodeOption{savemem}
\DeclareUnicodeOption{document}
\SetUnicodeOption[1000]{document}
\DeclareUnicodeOption{default}
\SetUnicodeOption[0]{default}
\XDeclareUnicodeOption{}{combine}{}{%
  \let\uc@cmb\empty}{%
  \ifx\unicodecombine\undefined\else\unicodecombine\fi
  \def\uc@cmb{\uc@warn@nocombine}}%
\ifx\AtBeginDocument\undefined\else
  \AtEndDocument{\unicodecombine}\fi
\SetUnicodeOption{nocombine}%
\def\uc@cmb{\uc@warn@nocombine}%
\ifx\DeclareOption\undefined\else
\DeclareOption{showmagickern}{\def\uc@magic@glue{6805678}}%
\DeclareOption{hyperref}{\AtEndOfPackage{\RequirePackage{ucshyper}}}%
\DeclareOption*{\SetUnicodeOption{\CurrentOption}}\ProcessOptions*
\fi
\ifx\AtBeginDocument\undefined
  \uc@warnmsg{Not loading ucsencs.def automatically.\MessageBreak
    Please load it after initializing fontencodings}%
\else
  \AtBeginDocument{\input{ucsencs.def}}\fi
\AtBeginDocument{\ifUnicodeOptiongraphics\RequirePackage{graphicx}\fi}%
\uc@newcommand\unicode@numtohex{\protect\unicode@numtohex@}%
\uc@newcommand\unicode@numtohex@#1#2#3{%
  {%\let\empty\relax\relax
   %\ifx\empty\relax\def\empty{}%
     \count255=#2\relax\gdef#1{}%
     \count252=#3%
     \loop
     \count253=\count252\advance\count253by\count255\relax
     \ifnum\count253>0%
     \ifnum\count252>0\advance\count252by-1\relax\fi
     \count254=\count255%
     \divide\count255by16%
     \multiply\count255by16%
     \advance\count254by-\count255%
     \xdef#1{\ifcase\count254 0\or1\or2\or3\or4\or5\or6\or7\or
       8\or9\or A\or B\or C\or D\or E\or F\fi#1}%
     \divide\count255by16\relax
     \repeat
   %\else
   %  \def#1{dec:#2}%
   %\fi
   }}
\let\uc@spc\space
\newcount\uc@secondtry
\uc@newcommand\unicode@invalid#1{%
  \unicode@combine%
  \ifUnicodeOptiongraphics{%
  \ifx\unicode@graphicsdir\undefined
    \def\unicode@graphicsdir{ucs-glyphs}\fi
  \ifx\unicode@graphicscmd\undefined
    \def\unicode@graphicscmd{ucs-getglyph \hex\space \dec\space \path\space}\fi
  \unicode@numtohex\hex{#1}4%
  \count255=#1\relax
  \divide\count255 by256\relax
  \unicode@numtohex\uc@temp@b{\count255}2%
  \edef\path{\unicode@graphicsdir/\uc@temp@b/U\hex.ps}%
  \edef\dec{\number#1}%
  \IfFileExists{\uc@temp@c}{}{%
    \typeout{Running: \unicode@graphicscmd}%
    \immediate\write18{\unicode@graphicscmd}%
    }%
 \IfFileExists{\path}{%
    \setbox255=\hbox{X}%
    \edef\uc@temp@b{\begingroup\noexpand\uni@resetcatcodes
      \noexpand\includegraphics[height=\the\ht255, trim=0 22.5 0 17.5]%
                      {\path}%
    \noexpand\ProvidesFile{U\hex.ps}%
        [Downloaded glyph for U+\hex]%
    \endgroup}%
  \typeout{\meaning\uc@temp@b}%
  \expandafter\unicodevirtual\expandafter{\uc@temp@b}%
  }{%
    \PackageWarning{ucs}{File \uc@temp@d\uc@temp@c.ps %SPACE
      not found.\MessageBreak
      Use\MessageBreak
      \space\space\space\space\unicode@graphicscmd\MessageBreak
      or start latex with option -shell-escape\MessageBreak
      if you have not already done so.}%
    \unicodevirtual{\unicode@invalidglyph{#1}}}}\else
    \unicodevirtual{\unicode@invalidglyph{#1}}\fi}
\uc@newcommand\unicode@invalidglyph#1{%
  {\unicode@numtohex\uc@temp@d{#1}4%
    \fontencoding{OT1}\texttt{[U+\uc@temp@d]}}}
\uc@newcommand\uni@char#1{%
  \ucs@protected@unichar\iftrue
    \expandafter\ifx\csname u-\number#1-h/o\endcsname\relax
  %    \end{macrocode}
  % If the character is not defined yet, load it.
  %    \begin{macrocode}
      \begingroup
        % In case \let is not executed, this (until ===) expands
        % to \let\relax\relax,
        % otherwise we have \let\uc@notloaderr\@gobble
        % Number of \empty's must equal number of args of \uc@char@notloaded
        \let\uc@notloaderr\@gobble\empty\@gobbletwo\relax\relax
        % ===
      \expandafter\endgroup
      % If \let not executed: Warning is emitted (see |\uc@notloaderr|)
      % otherwise: |\uc@char@notloaded| is called.
      \uc@notloaderr{\number#1}\uc@char@notloaded{#1}%
    \else
  %    \end{macrocode}
  % If the character is loaded, run |\uc@checkopts|
  % with the options of this character
  % as first arg and the code position as second; this will
  % display the character with
  % the correct option.
  %    \begin{macrocode}
     \expandafter\expandafter\expandafter\uc@checkopts
       \expandafter\expandafter\expandafter
       {\csname u-\number#1-h/o\endcsname}{#1}%
    \fi
  \else
    \noexpand\unichar{#1}%
  \fi
}
\begingroup
  \lccode`\A=`\{\lccode`\B=`\}\lccode`\C=`\\%
  \lccode`\P=`\P\lccode`\U=`\U%
  \lowercase{%
\endgroup
  \uc@newcommand\uc@notloaderr#1#2#3{%
    \ifx\@gobble#1\else[Please insert %SPACE
      CPrerenderUnicodeACunicharA#1BB into preamble]\fi}}
\uc@newcommand\uc@checkopts#1#2{%
  \expandafter\uc@checkopt@error\expandafter{\number#2}%
    {error}{error}{infinity}#1\@nil
}
\expandafter\uc@newcommand\csname uo-prio-infinity\endcsname{-2100000000}
%% === BEGIN AUTOGENERATED CODE
\uc@newcommand\uc@checkopt@stick#1#2#3#4#5{%
  \ifx\@nil#5%
\expandafter\ifx\csname u-#2-#1\endcsname\relax
  \uc@localdeferr{#1}{#2}%
\else
  \uc@output{\csname u-#2-#1\endcsname}{#1}%
\fi
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#2\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@stick
      \else
        \ifnum\csname uo-prio-#2\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@stick
    \fi
  \fi
  {#1}{#2}{#5}{#2}%
}
\uc@newcommand\uc@checkopt@change#1#2#3#4#5{%
  \ifx\@nil#5%
\expandafter\ifx\csname u-#3-#1\endcsname\relax
  \uc@localdeferr{#1}{#3}%
\else
  \uc@output{\csname u-#3-#1\endcsname}{#1}%
\fi
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#3\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@stick
      \else
        \ifnum\csname uo-prio-#3\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@stick
    \fi
  \fi
  {#1}{#3}{#5}{#3}%
}
\uc@newcommand\uc@checkopt@error#1#2#3#4#5{%
  \ifx\@nil#5%
\uc@errordrawopt{#1}{#2, #3}{#4}%
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#4\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@errorstick
      \else
        \ifnum\csname uo-prio-#4\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@errorstick
    \fi
  \fi
  {#1}{#2, #3}{#5}{#4}%
}
\uc@newcommand\uc@checkopt@errorstick#1#2#3#4#5{%
  \ifx\@nil#5%
\uc@errordrawopt{#1}{#2}{#4}%
    \expandafter\@gobblefour
  \else
    \iftrue\csname fi\endcsname
    \csname ifUnicodeOption#5\endcsname
      \ifnum\csname uo-prio-#4\endcsname>\csname uo-prio-#5\endcsname\uc@spc
        \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
        \uc@checkopt@errorstick
      \else
        \ifnum\csname uo-prio-#4\endcsname<\csname uo-prio-#5\endcsname\uc@spc
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@change
        \else
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter
          \uc@checkopt@error
        \fi
      \fi
    \else
      \expandafter\expandafter\expandafter\uc@checkopt@errorstick
    \fi
  \fi
  {#1}{#2}{#5}{#4}%
}
\let\unicode@empty\empty
\uc@newcommand\uc@errordrawopt#1#2#3{%
  \let\unicode@empty\relax\relax
  \ifx\unicode@empty\relax\let\unicode@empty\empty
    \unicode@numtohex\uc@temp@b{#1}4%
    \ifnum\csname uo-prio-#3\endcsname=-2100000000\relax
      \expandafter\ifx\csname
        missing-unicode-warned-\number#1\endcsname\relax
        \global\expandafter\let\csname
          missing-unicode-warned-\number#1\endcsname\@ne
        \unicode@error@unknown\@ne{Character \number#1\uc@spc
          \uc@spc= U+\uc@temp@b\uc@spc
          matches no activated options.\MessageBreak
          Type H to see available options}{#1}%
      \else
        \PackageWarning{ucs}{Character % SPACE
          \number#1 \uc@spc= 0x\uc@temp@b\uc@spc
          appeared again.}%
      \fi
    \else
      \@getcharinfo\uc@temp@c{#1}%
      \PackageWarning{ucs}{Character %SPACE
        \number#1 \uc@spc= 0x\uc@temp@b\uc@spc
        matches options\MessageBreak
        \uc@spc\uc@spc\uc@spc#2\MessageBreak
        with same priority \csname uo-prio-#3\endcsname. %SPACE
        Selecting option #3.\MessageBreak
        \uc@temp@c}%
      \uc@output{\csname u-#3-#1\endcsname}{#1}%
    \fi
  \else
    \noexpand\unichar{#1}%
  \fi
}
\uc@newcommand\uc@output#1#2{%
  \ifx\unicode@delay1\let\unicode@delay\relax\else
    \ifUnicodeOptioncombine
      \expandafter\uc@combine\expandafter{#1}{#2}%
    \else
      \uc@prechar@exec{#2}%
        \unicode@charfilter{#1{}}%
    \fi
    \ifx\uc@throw\undefined\else
      \def\uc@got{#2}\uc@throw\global\let\uc@throw\undefined\fi
  \fi
}%
\uc@newcommand\uc@prechar@exec#1{%
  \ifx\uc@prechar\undefined\else\uc@prechar{#1}\fi}
\uc@newcommand\uc@localdeferr#1#2{%
  \@getcharinfo\uc@temp@a{#1}%
  \PackageError{ucs}{Internal error in character \number#1, %SPACE
    option #2}{I probably got confused by intermixed local %SPACE
    and global definitions.\MessageBreak Try to load the needed %SPACE
    code page via \noexpand\PreloadUnicodePage
    before declaring anything by yourself.}{\uc@temp@a}%
  \unicode@invalid{#1}%
}%
\uc@newcommand\uc@warn@nocombine{%
  \PackageError{ucs}{Please activate option 'combine'}{Composed %SPACE
    characters can only be rendered correctly, when the option %SPACE
    'combine' is activated}}
\newtoks\uc@combtoks
\newtoks\uc@combtoksb
\newtoks\uc@temptokena
\uc@newcommand\unicode@combine{%
  \uc@check@magicglue%
  \ifx\uc@combining@prechar\undefined\global\let\uc@comb@code\undefined\fi
  \ifx\uc@comb@code\undefined\uc@temptokena{}\else
    \uc@temptokena\expandafter{\expandafter\uc@prechar@exec
      \expandafter{\uc@comb@code}}\fi%
  \global\let\uc@comb@code\undefined
  \global\expandafter\expandafter\expandafter\expandafter\expandafter
  \expandafter\expandafter\uc@combtoksb
  \expandafter\expandafter\expandafter
  \expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\the
    \expandafter\expandafter\expandafter\uc@combtoksb
    \expandafter\the\expandafter\uc@temptokena\the\uc@combtoks}%
  \global\uc@combtoks{}}
\def\uc@magic@glue{5381}
\uc@newcommand\uc@check@magicglue{%
  \ifnum\lastskip=\uc@magic@glue\unskip\else
    \begingroup
      \edef\uc@temp@a{\the\uc@combtoks}%
      \ifx\uc@temp@a\empty\else
      \PackageWarning{ucs}{Magic kern expected. Probably some %SPACE
        non-unicode characters mixed in while option combine was %SPACE
        in effect.}\fi\endgroup
  \fi}
\uc@newcommand\unicodevirtual#1{%
  \def\uc@temp@a##1{#1}\uc@output{\csname uc@temp@a\endcsname}{"FFFF}}
\uc@newcommand\unicodecombine{%
  \ifx\protect\@typeset@protect
    \unicode@combine%
    %\typeout{WRITING: \the\uc@combtoksb}%
    \the\uc@combtoksb
    \uc@prechar@exec{-1}%
    \global\uc@combtoksb{}%
      \ifx\uc@throw\undefined\else
        \def\uc@got{-1}\uc@throw\global\let\uc@throw\undefined\fi
  \else
    \noexpand\unicodecombine\fi
}
\uc@newcommand\uc@combine#1#2{%
  \ifx\protect\@typeset@protect
    \@temptokena\expandafter{#1{}}%
    \expandafter\expandafter\expandafter\ifx
    \expandafter\uc@firstofmany\the\@temptokena\uc@firstofmany\uc@cmb
      \uc@check@magicglue%
      \uc@combtoks\expandafter\expandafter\expandafter\expandafter
     \expandafter\expandafter\expandafter{%
        \expandafter\expandafter\expandafter\@gobble
        \expandafter#1\expandafter{\the\uc@combtoks}}%
    \else
      \unicode@combine%
      \xdef\uc@comb@code{\number#2}%
      \global\uc@combtoks\expandafter{#1{}}%
    \fi
    %\typeout{->COMBTOKS: \the\uc@combtoks}%
    \hskip\uc@magic@glue spplus0ptminus0pt %SPACE ; Insert magic glue
  \else
    \noexpand\unichar{\number#2}\fi
}
\uc@newcommand\uc@char@notloaded#1{%
  \count255=#1\divide\count255 by 256%
  \edef\uc@temp@a{uni-\number\count255.def}%
  \expandafter\ifx\csname\uc@temp@a\endcsname\relax\else
    \uc@secondtry#1\relax\fi
  \ifnum\uc@secondtry=#1\relax
    % If the file has already been loaded, but the character is unknown,
    % output an error and show the replacement glyph
    \unicode@numtohex\uc@temp@b{#1}4%
    \expandafter\ifx\csname
      missing-unicode-warned-\number#1\endcsname\relax
    \global\expandafter\let\csname
      missing-unicode-warned-\number#1\endcsname\@ne
      \unicode@error@unknown\@ne{Unknown Unicode character % SPACE
        \number#1 \uc@spc= U+\uc@temp@b,\MessageBreak
        possibly declared in \uc@temp@a.\MessageBreak
        Type H to see if it is available with options}{#1}%
    \else
      \PackageWarning{ucs}{Unknown character % SPACE
        \number#1 \uc@spc = 0x\uc@temp@b\uc@spc
        appeared again.}%
      \unicode@invalid{#1}%
    \fi
  \else
    \begingroup
    \ifUnicodeOptionsavemem
    \else
      \global\expandafter\let\csname\uc@temp@a\endcsname\@ne
    \fi
    \def\uc@got{#1}%
    \uni@resetcatcodes
    \expandafter\InputIfFileExists\expandafter{\uc@temp@a}{%
      \global\let\uni@dataloaded1%
      }{%
      }%
      % End of local group for inputted file
    \endgroup
      % Retry displaying character. This won't cause infinite recursion,
      % because we have marked this file as loaded (globally or, if
      % |savemem| is set, at least here).
    \uc@secondtry#1\relax%
    \uni@char{#1}%
  \fi
  }
\uc@newcommand\PreloadUnicodePage#1{%
  \begingroup
  \global\expandafter\let\csname uni-#1.def\endcsname\@ne
  \uni@resetcatcodes
  \InputIfFileExists{uni-#1.def}{\let\uni@dataloaded1}{%
    \PackageError{ucs}{Could not find uni-#1.def}{}}%
  \endgroup}
\uc@newcommand\PrerenderUnicode{%
  \@ifstar{\@prerenderunicode\unichar}{\@prerenderunicode\@gobble}}%
\uc@newcommand\@prerenderunicode#1#2{%
  \begingroup
  \UnicodeCharFilter\@gobble
  \let#1\@gobble\setbox0\hbox{#2}\endgroup}
\uc@newcommand\DeclareUnicodeCharacter#1#2{%
  \DeclareUnicodeCharacterAsOptional{#1}{document}{#2}}
\uc@newcommand\DeclareUnicodeCharacterAsOptional{%
  \let\uc@temp@a\relax\uni@declcharopt}
\uc@newcommand\uc@dclc#1#2{%
  \let\next=\uni@declcharopt
  \ifUnicodeOptionsavemem
    \ifnum\uc@got=#1\else
      \let\next=\@gobblethree\fi
  \fi
  \ifx\next\uni@declcharopt
    \expandafter\ifx\csname uni@active@#2\endcsname\relax
      \let\next\@gobblethree\else
    \expandafter\ifx\csname u-#2-\number#1\endcsname\relax\else
      \let\next\@gobblethree\fi\fi
    \let\uc@temp@a\global
  \fi
  \next{#1}{#2}}
\uc@newcommand\uni@declcharopt#1#2#3{%
  %\typeout{Defining: u-#2-\number#1 (\meaning\uc@temp@a)}%
  \ifx\utf@viii@map\undefined\else
    \expandafter\utf@viii@map\expandafter{\number#1}\fi
  \expandafter\uc@temp@a\expandafter\def
    \csname u-#2-\number#1\endcsname##1{#3}%\fi
  \expandafter\ifx\csname u-\number#1-h/o\endcsname\relax
    \expandafter\def\csname u-\number#1-h/o\endcsname{}\fi
  \expandafter\uc@temp@a\expandafter\edef
    \csname u-\number#1-h/o\endcsname{%
    {#2}\csname u-\number#1-h/o\endcsname}%
  }%
\let\unichar\uni@char
\uc@newcommand\unicodesuper#1{\textsuperscript{#1}}%
\uc@newcommand\@getcharinfo#1#2{%
  \begingroup
  \countdef\uc@got0\relax\uc@got#2\relax
  \global\def#1{Character's name unknown}%
  \def\info##1{\xdef#1{##1}}%
  \uni@resetcatcodes
  \ifUnicodeOptionfasterrors
  \global\def#1{No further informations known % SPACE
    because of option fasterrors.}\else
  {\InputIfFileExists{uninames.dat}{}{%
    \global\def#1{Character database uninames.dat not found. %SPACE
      \MessageBreak Character \number#2 \uc@spc unknown}}}%
  \fi
  \toks255{}%
  \def\uc@dclc##1##2##3{\ifnum##1=\uc@got
    \toks255\expandafter{\the\toks255, ##2}\fi}%
  \count255\uc@got\divide\count255by256\relax
  %\edef\temp@a{uni-\number\count255.def}%
  \InputIfFileExists{uni-\number\count255.def}{}{}%
  \expandafter\ifx\expandafter\@nil\the\toks255 \@nil
    \xdef#1{#1\noexpand\MessageBreak
      Character is not defined in uni-*.def files}%
  \else
    \expandafter\expandafter\expandafter\@getcharinfo@
    \expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter
    {\expandafter#1\expandafter}\the\toks255 \@nil%
  \fi
  \endgroup}
\def\@getcharinfo@#1#2, #3\@nil{\gdef#1{#2\MessageBreak
    Character available with following options:\MessageBreak
    \uc@spc\uc@spc\uc@spc #3}}
\uc@newcommand\PrintUnicodeName#1{{%
  \@getcharinfo{\ci}{#1}%
  \def\MessageBreak{^^J}%
  \typeout{^^J\ci^^J}}}
\uc@newcommand\UnicodeCharFilter#1{\let\unicode@charfilter=#1}
\uc@newcommand\UCSProtectionNone{%
  \def\ucs@protected@unichar{}%
  \UnicodeCharFilter\@firstofone}
\uc@newcommand\UCSProtectionIeC{%
  \def\ucs@protected@unichar{}%
  \UnicodeCharFilter\IeC}
\uc@newcommand\UCSProtectionUnichar{%
  \def\ucs@protected@unichar##1{\ifx\protect\@typeset@protect}%
  \UnicodeCharFilter\@firstofone}
\UCSProtectionIeC
\uc@newcommand\uni@resetcatcodes{%
  \endlinechar=13\relax
  \def\reserved@a##1##2{%
    \@tempcnta##1\relax
    \@tempcntb##2\relax
    \reserved@b
    }%
  \def\reserved@b{%
    \ifnum\@tempcnta>\@tempcntb\else
    \reserved@c\@tempcnta
    \advance\@tempcnta\@ne
    \expandafter\reserved@b
    \fi
    }%
  \catcode`\ =10\relax
  \catcode`\#=6\relax
  \catcode`\$=3\relax
  \catcode`\%=14\relax
  \catcode`\&=4\relax
  \catcode`\\=0\relax
  \catcode`\^=7\relax
  \catcode`\_=8\relax
  \catcode`\{=1\relax
  \catcode`\}=2\relax
  \catcode`\~=13\relax
  \catcode`\@=11\relax
  \catcode`\^^I=10\relax
  \catcode`\^^J=12\relax
  \catcode`\^^L=12\relax
  \catcode`\^^M=5\relax
  \def\reserved@c##1{\catcode##1=12\relax}%
  \reserved@c{`\!}%
  \reserved@c{`\"}%
  \reserved@a{`\'}{`\?}%
  \reserved@c{`\[}%
  \reserved@c{`\]}%
  \reserved@c{`\`}%
  \reserved@c{`\|}%
  \def\reserved@c##1{\catcode##1=11\relax}%
  \reserved@a{`\A}{`\Z}%
  \reserved@a{`\a}{`\z}%
  \def\reserved@c##1{\catcode##1=15\relax}%
  \reserved@a{0}{`\^^H}%
  \reserved@c{`\^^K}%
  \reserved@a{`\^^N}{31}%
  \catcode"7F=15\relax
  \relax}
\catcode`\!13\relax
\uc@newcommand\unicode@error@unknown{\protect\unicode@error@unknown@}%
\uc@newcommand\unicode@error@unknown@#1#2#3{%
  {\expandafter\countdef\expandafter\uc@got\expandafter0%
     \expandafter\relax\expandafter\uc@got\number#3\relax
  \ifx\measuring@false\undefined\else\measuring@false\fi
  \@getcharinfo\uc@temp@c{#3}%
  \ifUnicodeOptionwarnunknown
    \PackageWarning{ucs}{#2\MessageBreak\uc@temp@c.\MessageBreak
        Enter I\noexpand!<RET> to define the glyph.}%
    \ifx#1\@ne\unicode@invalid{#3}\fi
  \else
    \let!\unicode@read@definition\catcode`\!13\relax
    \let\uc@read@definition\undefined
    \PackageError{ucs}{#2}{\uc@temp@c.\MessageBreak
        Enter I\noexpand!<RET> to define the glyph.}%
    \ifx#1\@ne
    \ifx\uc@read@definition\undefined\unicode@invalid{#3}%
    \else\uc@read@definition\fi\fi
  \fi}}
\catcode`\!12\relax
\uc@newcommand\unicode@read@definition{%
  \uni@resetcatcodes
  \typein[\definition]{Please enter definition for %SPACE
    unicode character \number\uc@got}%
  \global\let\uc@read@definition\definition
  \toks255\expandafter{\definition}%
  \edef\definition{\noexpand\DeclareUnicodeCharacter%
    {\number\uc@got}{\the\toks255}}%
  \toks255\expandafter{\definition}%
  \typeout{Tip:\MessageBreak You may include\MessageBreak
    \uc@spc\uc@spc\the\toks255\MessageBreak
    into your document source.}%
  \the\toks255\relax
  }
\def\uc@firstofmany#1#2\uc@firstofmany{#1}
\ifx\AtBeginDocument\undefined\else
\AtBeginDocument{\def\uc@tempa{\@inpenc@undefined@{utf8}}%
  \ifx\@inpenc@undefined\uc@tempa
  \ifx\restore@utf@viii@actives\undefined
  \PackageWarning{ucs}{***************************\MessageBreak You %SPACE
    seem to have loaded inputencoding utf8\MessageBreak (LaTeX kernel %SPACE
    UTF-8) instead of utf8x (ucs.sty UTF-8).\MessageBreak Probably you %SPACE
    are compiling a document written for a\MessageBreak
    pre-august-2004 ucs.sty.\MessageBreak
    ***************************\MessageBreak Please use %SPACE
    \string\usepackage[utf8x]{inputenc} instead of\MessageBreak
    \string\usepackage[utf8]{inputenc}.\MessageBreak
    ***************************\MessageBreak If you should really want %SPACE
    to use ucs.sty and kernel's\MessageBreak utf8.def together, use %SPACE
    \string\usepackage[utf8x,utf8]{inputenc}\MessageBreak to disable %SPACE
    compatibility mode\MessageBreak
    ***************************\MessageBreak Activating compatibility %SPACE
    mode.\MessageBreak ***************************\MessageBreak}%
  \global\let\uc@inputencoding\inputencoding
  \inputencoding{utf8x}%
  \def\inputencoding#1{%
    {\def\uc@tempa{#1}\def\uc@tempb{utf8}\ifx\uc@tempa\uc@tempb
      \aftergroup\@firstoftwo\else\aftergroup\@secondoftwo\fi}%
    {\restore@utf@viii@actives}{\uc@inputencoding{#1}}}%
  \fi\fi
}\fi

